Common Neighborhood Estimation over Bipartite Graphs under Local Differential Privacy

Bipartite graphs, formed by two vertex layers, arise as a natural fit for modeling the relationships between two groups of entities. In bipartite graphs, common neighborhood computation between two vertices on the same vertex layer is a basic operator, which is easily solvable in general settings. However, it inevitably involves releasing the neighborhood information of vertices, posing a significant privacy risk for users in real-world applications. To protect edge privacy in bipartite graphs, in this paper, we study the problem of estimating the number of common neighbors of two vertices on the same layer under edge local differential privacy (edge LDP). The problem is challenging in the context of edge LDP since each vertex on the opposite layer of the query vertices can potentially be a common neighbor. To obtain efficient and accurate estimates, we propose a multiple-round framework that significantly reduces the candidate pool of common neighbors and enables the query vertices to construct unbiased estimators locally. Furthermore, we improve data utility by incorporating the estimators built from the neighbors of both query vertices and devise privacy budget allocation optimizations. These improve the estimator's robustness and consistency, particularly against query vertices with imbalanced degrees. Extensive experiments on 15 datasets validate the effectiveness and efficiency of our proposed techniques.

==> 8ack.tex <==
\section{Acknowledgments}
\label{acknowledgment}
% Kai Wang and Xuemin Lin are supported by NSFC U2241211. 
% Wenjie Zhang is supported by ARC FT210100303. 
% Ying Zhang is supported by ARC DP210101393 and DP230101445. 
% This work was partially supported by NSFC U2241211, ARC FT210100303, ARC DP210101393, and ARC DP230101445. 
% We would like to thank the anonymous reviewers for their valuable and constructive feedback. 
Kai Wang is the corresponding author.
Kai Wang is supported by NSFC 62302294 and U2241211. 
\textcolor{red}{Wenjie Zhang is supported by ARC DP230101445 and FT210100303.} 
Xuemin Lin is supported by NSFC U2241211. 
\textcolor{red}{Ying Zhang is supported by ARC DP210101393, LP210301046, and DP230101445.} 
We would like to thank the anonymous reviewers for their valuable and constructive feedback. 

==> abs.tex <==
Bipartite graphs, represented by two vertex layers, arise as a natural fit for modeling the relationships between two groups of entities. In bipartite graphs, common neighborhood computation between two vertices on the same vertex layer is a basic operator, which is easily solvable in general settings. However, it inevitably involves releasing the neighborhood information of vertices, posing a significant privacy risk for users in real-world applications. To protect edge privacy in graphs, in this paper, we study the problem of estimating the number of common neighbors of two vertices on the same layer on bipartite graphs under edge local differential privacy (edge LDP). The problem is challenging in the context of edge LDP since each vertex on the opposite layer of the query vertices could potentially be a common neighbor. To obtain efficient and accurate estimates, we propose a multiple-round framework that significantly reduces the candidate pool of common neighbors and enables the query vertices to construct unbiased estimators locally. Furthermore, we improve data utility by incorporating the estimators built from the neighborhoods of both query vertices and devise privacy budget allocation optimizations. These improve the estimator's robustness and consistency, particularly against query vertices with imbalanced degrees. Extensive experiments on 16 datasets validate the effectiveness and efficiency of our proposed techniques.

==> bkp3hop.tex <==
% \section{3 hop neighborhood exploration}


\section{ Extending to k-hop neighbors }

If we want to find $f_3(q, x)$, then it is unfortunate that we cannot leverage the $f(q, x)$, the number of two-hop paths, for this task. Because we cannot just aggregate the $f_2$ of the neighbor of $q$ and expect $f_3$, which results in duplicates. 

If we directly consider a query-vertex-centric approach for $f_3$ estimation. 

$$
\Tilde{f_3}(q, x) = \sum_{u \in N(q, G)} \sum_{ \substack{v \neq u \\ v \neq q \\ v \neq x   }} \phi'(u,v) \phi'(v,x)
$$

This is also unbiased. Its global sensitivity however becomes: 

$$
\Delta(\Tilde{f}_3) \leq \sum_{ \substack{v \neq u \\ v \neq q \\ v \neq x   }} \phi'(u,v) \phi'(v,x)
\leq (\frac{1-p}{1-2p})^2(n-3)
$$

The variance becomes impossible to compute due to the correlations of two-hop paths. 




\section{Experimental evaluation}
\label{sec:exp}




Algorithms: 

\begin{enumerate}
\item the naive algorithm: directly compute f vector on the noisy graph 
\item baseline algorithm: one-round algorithm
\item adv algorithm: two-round algorithm
\end{enumerate}


\noindent
{\bf Parameters.} 
Privacy budget epsilon. For two-round algorithms, we can visualize the effect of different privacy budget allocation. 


\noindent
{\bf Performance metric.} 
\begin{enumerate}
    \item Given a query vertex q, we compute the L1-loss of the f2 vector. 
    \item Given a query q, we compute the coverage of two-hop neighbours of the vertices with the top-K f2-values. 
    (the second one don't even need to be done)
\end{enumerate}



\noindent
{\bf Experiments.} 


\begin{enumerate}
    \item Default queries: 
For each graph, randomly sample 100 query vertices.  Then, we compute the f2 vector. Based on this, we compute the L1-loss or L2-loss. We report the average loss across the sampled vertices. 

\item The time and communication cost of different algorithms. 

\item Effect of privacy budget 
\begin{itemize}
    \item The effect of varying privacy budget on Naive, BS, and ADV on the L1-loss of f2-vector 
    % issue: how do we evaluate the relative error when the true value is zero? 
    % \item The effect of varying privacy budget on the three algorithms on the two-hop neighbor coverage. 
\end{itemize}
% (Issue: how do we determine the number of vertices to take? The size of K?)
% Is there a way for us to predict the size of the two-hop neighborhood? 

\item Evaluate of the effect of query vertex degree 
Sample high-degree and low-degree vertices.  Observe and explain the performance difference. 

\item 
 For two rounds: we evaluate the effectiveness of our privacy budget allocation technique. 
We can find that the budget allocation plan computed is indeed minimising the variance. 

\end{enumerate}





\subsection{Application scenarios}

\noindent
{\bf Papers directly using one-mode projection. }
Polarity‑based graph neural network for sign prediction in signed bipartite graphs \cite{zhang2022polarity}, Bipartite graph capsule network \cite{zhang2023bipartite}, ``Efficient High-quality Clustering for Large Bipartite Graphs'' \cite{yang2023efficient}. These papers directly project bipartite graphs into a homogeneous graph with edge weight. The weight is computed as the number of two-hop-paths between two vertices on the same layer. 


% Efficient High-quality Clustering for Large Bipartite Graphs (edge weighted)
\noindent
{\bf Papers intra-domain message passing: }
L-BGNN: Layerwise Trained Bipartite Graph Neural Networks \cite{xie2022bgnn}. 


\noindent
{\bf Papers using number of two-hop paths to model node similarity:}
``Scalable and effective bipartite network embedding'' \cite{yang2022scalable}. 
For u and x, it considers all paths of even length between them to formulate node proximity. We know that the number of even length path can be obtained once the length-2 paths are obtained. 

\noindent
{\bf Papers using two-hop neighbors on non-GNN tasks:}
biclique counting \cite{qiu2024accelerating}

% Qiu, Linshan, et al. "Accelerating Biclique Counting on GPU." arXiv preprint arXiv:2403.07858 (2024).
% biclique counting: tau-strengthened two-hop neighbours. Arguably will benefit pqbiclique counting under edge LDP





% $\phi_3(q, x) = 1$ if there exists a path of length 3 from $q$ to $x$, and 0 otherwise.

% $$
% \phi_k(q, x) = \begin{cases} 
% 1 & \text{there exists a path of length $k$ from } q \text{ to } x \\
% 0 & \text{otherwise}
% \end{cases}
% $$

% $$
% \phi_3(q, x) = 1 - \prod_{v_1, v_2}(1 - y_3(q, v_1, v_2, x))
% $$

% Equivalently, using logical operators:
% $$
% \phi_3(q, x) = \neg \left( \bigwedge_{v_1, v_2} \neg y_3(q, v_1, v_2, x) \right)
% $$

% We explore non-interactive and interactive solutions for this. 

% When $k = 3$, the above approaches present some difficulties. 
% First, we no longer have the formula for the expected value of $\phi_3$ any more. Even if we have unbiased estimates of all $y_3(q, v_1, v_2, x)$, we cannot use them to compute $\phi_3(q, x)$ because these paths of length $3$ overlap with each other, causing them to be not independent. When these terms are not independent, we cannot substitute the formula for unbiased estimates of $y_3$ and yield the estimator for $\phi_3$. 

% {\color{blue}
% If we directly substitute $y$ into the formula, we can argue that the expected value of the products is larger than the product of the expected values, given that the variables are positively correlated. 
% }


% The absolute values of $\phi_2$ and $\phi_3$ has the following relationship: 
% $$
% \phi_3(q, x) = 1 - \prod_{x' \in N(x, G)} (1- \phi_2(q, x'))
% $$



% Question: if we have a good estimate of $\phi_2(q, x)$, can we use it to estimate $\phi_3(q, x)$ in an unbiased manner? 


==> tabcomplexity.tex <==
\begin{table}[tbh]
\centering
\caption{Summary of time costs and expected L2 losses}
\myspace
\scalebox{0.9}{
\begin{tabular}{c|c|c|c} 
\noalign{\hrule height 1pt}
\cellcolor{gray!25} Algorithm   & \cellcolor{gray!25} Time cost &  \cellcolor{gray!25} Unbiased & \cellcolor{gray!25} expected L2 loss\\
\noalign{\hrule height 0.56pt}
\naive    & $O( n')$ & $\times$  & $ O( \frac{n'^2}{(1+e^{\varepsilon})^4}) $  \\
\bs       & $O(n')$  & \checkmark & $  O(\frac{ n'  e^{\varepsilon}}{(1 - e^{\varepsilon})^4} )  $  \\
\advss  & $O(n')$ & \checkmark & $  O(\frac{ e^{\varepsilon_1}}{(1 - e^{\varepsilon_1})^2} (d_u + \frac{ 2 e^{\varepsilon_1}}{\varepsilon_2^2} ) )$   \\
\advds  & 
$O(n)$ & \checkmark & 
\makecell{
$O(\frac{e^{\varepsilon_1}}{(1 - e^{\varepsilon_1})^2} (\alpha^2 d_u + (1-\alpha)^2 d_w)+ $ \\
$
\frac{2 e^{2\varepsilon_1}}{(1 - e^{\varepsilon_1})^2} 
\frac{\alpha^2 + (1-\alpha)^2 }{\varepsilon_2^2} )$
\vspace{0.2mm}
}
\\
\noalign{\hrule height 1pt}
\end{tabular}
}
\begin{flushleft}
* $\varepsilon$ is the overall privacy budget. 
% In \advss and \advds, $\varepsilon_1$ and $\varepsilon_2$ denote the privacy budget for randomized responses and the Laplace mechanism, respectively. 
 In \advss and \advds, $\varepsilon_1$ represents the privacy budget for randomized responses, while $\varepsilon_2$ denotes the budget for the Laplace mechanism. 
 $\alpha \in [0,1]$ adjusts the contribution of $\fq$ and $\fx$. 
% $\varepsilon_2$ denotes the privacy budget for the Laplace mechanism, in \advss and \advds. 
$d_u$ and $d_w$ represent the degrees of $u$ and $w$ in $G$. 
$n'$ denotes the number of vertices on the opposite layer of $u$ and $w$. 
$n$ denotes the number of all vertices in $G$. 
% $G_{\varepsilon}'$ denotes a noisy graph w.r.t. $\varepsilon$. 
% $n_1$ and $n_2$ denotes the number of upper and lower vertices, resp. 
\end{flushleft}
\label{tab:complexitycompare}
\end{table}

==> time-tab.tex <==
\begin{table}
    \centering
\caption{The running time (sec) xxx}
\label{tab:dataset_results}
\begin{tabular}{l| rrrr}
\toprule
Dataset & Naive & Bs & Adv1 & Adv2 \\
\midrule
rmwiki & 0.031 & 0.031 & 0.042 & 0.041 \\
opsahl-collaboration & 0.066 & 0.066 & 0.087 & 0.085 \\
occupation & 0.312 & 0.314 & 0.488 & 0.388 \\
location & 0.371 & 0.373 & 0.566 & 0.479 \\
bag-kos & 0.033 & 0.033 & 0.043 & 0.041 \\
bpywiki & 0.105 & 0.105 & 0.143 & 0.141 \\
tewiktionary & 0.903 & 0.904 & 0.994 & 0.978 \\
bookcrossing & 0.899 & 0.907 & 1.216 & 1.091 \\
stackoverflow & 1.325 & 1.332 & 1.788 & 1.470 \\
dbpedia-team & 2.365 & 2.382 & 3.024 & 2.767 \\
digg-votes & 2.514 & 2.516 & 2.700 & 2.631 \\
wiki-en-cat & 4.991 & 5.026 & 5.948 & 5.640 \\
movielens & 1.202 & 1.202 & 1.248 & 1.215 \\
epinions & 2.285 & 2.303 & 2.654 & 2.555 \\
netflix & 56.905 & 56.905 & 59.559 & 59.234 \\
delicious-ui & 226.757 & 227.492 & 229.040 & 218.665 \\
orkut & 61.165 & 61.248 & 57.934 & 55.084 \\
\bottomrule
\end{tabular}
\end{table}
